COOL-MC: A Comprehensive Tool for Reinforcement Learning and Model Checking

This paper presents COOL-MC, a tool that integrates state-of-the-art reinforcement learning (RL) and model checking. Specifically, the tool builds upon the OpenAI gym and the probabilistic model checker Storm. COOL-MC provides the following features: (1) a simulator to train RL policies in the OpenAI gym for Markov decision processes (MDPs) that are defined as input for Storm, (2) a new model builder for Storm, which uses callback functions to verify (neural network) RL policies, (3) formal abstractions that relate models and policies specified in OpenAI gym or Storm, and (4) algorithms to obtain bounds on the performance of so-called permissive policies. We describe the components and architecture of COOL-MC and demonstrate its features on multiple benchmark environments.

==> atva_benchmarks.tex <==

\begin{table}[t]
\scalebox{0.85}{
\begin{tabular}{|l|l|r|r|r|r|r|}
\hline
Environment     & Specification                                            & Result & Building Time & Checking Time & States & Transitions \\ \hline
Frozen Lake     & $\mathcal{P}^{\pi_A}(\lozenge water)$                              & 0.18                  & 0.25                & 0                   & 14               & 34                    \\ \hline
Taxi            & $\mathcal{P}^{\pi_C}(\lozenge empty)$      & 0                     & 4.78                & 0                   & 252              & 507                   \\ \hline
Taxi            & $\mathcal{P}^{\pi_C}(\lozenge done=2)$      & 1                     & 4.5                & 0                   & 252              & 507                   \\ \hline
Collision $5\times5$   & $\mathcal{P}^{\pi_D}_{\leq 100}(\lozenge collide)$                     & 0.25                  & 44                 & 0.47                & 15133            & 212289                \\ \hline
Collision $6\times6$   & $\mathcal{P}^{\pi_D}_{\leq 100}(\lozenge collide)$                     & 0.19                  & 142                 & 1.58                & 45496            & 662395                \\ \hline
Collision $7\times7$  & $\mathcal{P}^{\pi_D}_{\leq 100}(\lozenge collide)$                   & 0.16                  & 357                 & 4.43                & 114278           & 1702341               \\ \hline
Collision $10\times10$ &$\mathcal{T}^{\pi_D}(\lozenge collide)$                        & 470.73                & 3106                & 226                 & 1000000          & 29256683              \\ \hline
Collision $11\times11$ &$\mathcal{T}^{\pi_D}(\lozenge collide)$                        & 546.18               & 3909                & 314                 & 1771561          & 52433826              \\ \hline
Collision $12\times12$ &$\mathcal{T}^{\pi_D}(\lozenge collide)$                        & FAILURE                & 6619                & FAILURE                 & 2985984          & 89198366              \\ \hline
Collision $16\times16$ &$\mathcal{T}^{\pi_D}(\lozenge collide)$                        & M/O                & M/O                & M/O                 & 17295388          & 2058859952              \\ \hline
Smart Grid      & $\mathcal{P}^{\pi_E}_{\leq 1000}(\lozenge blackout)$            & 0.02                  & 0.48                & 0                   & 40               & 176                   \\ \hline
Stock Market    & $\mathcal{P}^{\pi_F}_{}(\lozenge bankruptcy)$ & 0                     & 0.3                 & 0                   & 130              & 377                   \\ \hline
Stock Market    & $\mathcal{P}^{\pi_F}_{}(\lozenge success)$ & 1                     & 0.19                 & 0                   & 53              & 147                \\ \hline
James Bond    & $\mathcal{P}^{\pi_G}_{\leq 15}(\lozenge done)$ & 0.23                     & 1997                 & 0.28                   & 159744              &   1105920             \\ \hline
Crazy Climber    & $\mathcal{P}^{\pi_H}_{\leq 15}(\lozenge done)$ & 0                    &   175               & 0                 & 8193             & 32772                \\ \hline
\end{tabular}
}



\end{table}

==> collision_avoidance_section.tex <==
\subsection{Collision Avoidance System}
Collision avoidance is an environment which contains one agent and two moving obstacles in a two dimensional grid world. The environment terminates as soon as a collision between the agent and one obstacle happens. The environment contains a slickness parameter, which defines the probability that the agent stays in the same cell.

\begin{align*} 
States = \{(x,y,obstacle\_x,obstacle\_y,obstacle\_x,obstacle\_y,done),...\} \\
Actions = \{NORTH,EAST,SOUTH,WEST\}\\
Reward = \begin{cases}
        0 \text{, if collision}
        \\
        100 \text {, otherwise}
        \end{cases}
\end{align*}
We trained a deep RL agent for $11,000$ epochs in a $4x4$ grid. This trained agent collides in average after 1041 steps into an obstacle. After creating a more abstract representation of the agent position representation (4x4 to 2x2), we get an average number of 220 steps until the collision. It is also possible to combine state abstraction and permissive model checking. The permissive policy for a sensor that combines two cells into one and ignoring the obstacle positions leads minimal after $7.4$ steps and maximal after $20028$ steps to a collision. If we instead combining two cells into one cell for the obstacle coordinations the agent runs into a collision of minimal $10$ steps and maximal $12976$ steps. 

%$Tmin=? [F COLLISION=true] : 7.444806505202438$
%$Tmax=? [F COLLISION=true] : 20028.08903963102$

%$Tmax=? [F COLLISION=true] : 10$
%$Tmax=? [F COLLISION=true] : 12976$

==> old_experiments.tex <==
\section{Experiments}
We analyze several environments with COOL-MC. We model check safety properties, worst-/best-case scenarios, and verify trained policies on more abstract states.
All the experiments were executed on a laptop with a NVIDIA GeForce GTX 1060 Mobile GPU, 8 GB RAM and an Intel(R) Core(TM) i7-8750H CPU @ 2.20GHz x 12.

{\color{red} we have to better explain what we are checking and why we are doing it, write it in PCTL everywhere}

\subsection{OpenAI Gym Policy Verification}
\iffalse
\begin{floatingfigure}{4cm}
\centering
\begin{tikzpicture}
    \draw[step=1cm,gray,very thin] (0,0) grid (4,4);
    \fill[yellow!100!white] (0,3) rectangle (1,4);
    \fill[blue!100!white] (0,0) rectangle (1,1);
    \fill[blue!100!Green] (1,2) rectangle (2,3);
    \fill[blue!100!white] (3,2) rectangle (4,3);
    \fill[blue!100!white] (3,1) rectangle (4,2);
    \fill[green!100!white] (4,1) rectangle (3,0);
    % Features
    \node[] at (0.5,3.5)
    {0};
    \node[] at (1.5,3.5)
    {1};
    \node[] at (2.5,3.5)
    {2};
    \node[] at (3.5,3.5)
    {3};
    \node[] at (0.5,2.5)
    {4};
    \node[] at (1.5,2.5)
    {5};
    \node[] at (2.5,2.5)
    {6};
    \node[] at (3.5,2.5)
    {7};
    \node[] at (0.5,1.5)
    {8};
    \node[] at (1.5,1.5)
    {9};
    \node[] at (2.5,1.5)
    {10};
    \node[] at (3.5,1.5)
    {11};
    \node[] at (0.5,0.5)
    {12};
    \node[] at (1.5,0.5)
    {13};
    \node[] at (2.5,0.5)
    {14};
    \node[] at (3.5,0.5)
    {15};

\end{tikzpicture}

\caption{Frozen Lake State. Start position (yellow), ice (white), water (blue), and frisbee (green).}

\end{floatingfigure}
\fi
\begin{floatingfigure}{6cm}
\centering
        \includegraphics[page=1,width=.45\textwidth]{frozen_lake_probs}
        %\scalebox{0.43}{\input{frozen_lake_probs}}
\caption{Frozen Lake State. Start position (0), water holes (5,7,11,12), and frisbee (15).}
\label{fig:frozen_lake}
\end{floatingfigure}
We show in this experiment that it is possible to train a RL policy in a OpenAI gym environment and verify its performance via model checking.
The \textit{frozen lake} environment is a commonly used OpenAI Gym benchmark, where 
the agent has to reach the goal (frisbee) on a frozen lake. The movement direction of the agent is uncertain and only depends in $33.33\%$ of the cases on the chosen direction. In $66.66\%$ of the cases, a neighbor action of the actual action is chosen (see neighbor actions in action space).  The environment terminates as soon as the agent falls into the water or reaches the goal state \cite{brockman2016openai}. Movements against the frozen lake edge lead to the same state, or the agent slips. The environment is defined as follows:
\begin{align*} 
States = \{0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15\} \\
Actions = \{UP, LEFT, DOWN, RIGHT\}\\
Reward = \begin{cases}
        1 \text{, if state = 15 (Frisbee).}
        \\
        0 \text {, otherwise}.
        \end{cases}
\end{align*}

First, we trained a deep RL agent on this frozen lake environment and received after $100,000$ episodes an average reward of $0.81$ over $100$ episodes. Since this reward value was empirically calculated, we wanted to quantify the trained agent properties on the environment formally.
Therefore, we modeled the frozen lake environment as an MDP via PRISM, which allowed us to query the actual probability of reaching the frisbee which is $Prob_{=0.82}(\lozenge frisbee)$. The probability for the agent to fall into the water is $Prob_{=0.18}(\lozenge water)$. A closer investigation showed that the agent only falls into the water hole at the fifth position (from $state=6$ while using the action $LEFT$). The agent reaches state $9$ with a probability of $Prob_{=1}(\lozenge 9)$. At this state, we split the environment into a safe and unsafe area. If the agent can successfully execute the $DOWN$ action, he stays safe the rest of the trajectory to the frisbee. Suppose the agent slips to state 10 while executing action $DOWN$, the probability of falling into the water hole increases to $Prob_{=0.24}(water)(10)$. From there, the only way to decrease the probability of falling into the water is by trying to go back to state $9$. So, at state $10$, the agent tries to execute action $LEFT$, which brings him, in the best case, back or to the most critical state (state $6$), which has a probability of $Prob_{=0.33}(water)(6)$.
This investigation also shows that the trained agent learned to take the slippery factor into account. If he just wanted to reach the frisbee, he would just have taken action $DOWN$, which brings him closer to the frisbee but has a higher probability of falling into the water.

\subsection{Permissive Model Checking}
In this experiment, we use permissive model checking to investigate the worst-~/best-case behaviour of the policy and analyze how a less precise sensor influence the trained policy performance (state abstraction).
In the \textit{Taxi} environment, the taxi agent has to pick up passengers and transport them to their destination without running out of fuel. The environment terminates as soon as the taxi agent does the predefined number of jobs. After the job is done, a new guest spawns randomly at one of the predefined locations based on a uniform distribution.
\begin{align*} 
States = \{(x,y,pickup\_x,pickup\_y,destination\_x,destination\_y,\\fuel,jobs\_done,on\_board),...\} \\
Actions = \{NORTH,EAST,SOUTH,WEST,PICK\_UP,DROP\}\\
Penalty = \begin{cases}
        0 \text{, if passenger successfully dropped.}
        \\
        21 \text {, if passenger got picked up.}
        \\
        21 + |x-dop\_x| + |x-dop\_y| \text {, if passenger on board.}
        \\
        21 + |x-pickup\_x| + |x-pickup\_y| \text {, otherwise}
        \end{cases}
\end{align*}
We trained our taxi agent for $75,000$ episodes on the taxi environment with an initial $MAX\_FUEL=10$ and two jobs $(MAX\_JOBS=2)$. The trained agent finishes all two jobs with a probability of $Prob_{=0.5625}(jobs\_done=2)$ and one job with a probability of $Prob_{=1}(jobs\_done=1)$ (the first job is always the same). This insight allowed us to retrain the agent to archive a $100\%$ probability of finishing two jobs after $125,000$ epochs. Figure \ref{fig:out_of_fuel} plots the likelihood of different properties. The x-axis defines the maximal fuel level, which can be sensored by the taxi agent and does not reflect the exact fuel level in the 10 level tank. The retrained agent outperforms the original agent in running out of fuel and finishing two jobs.
With permissive model checking, we plot the worst-/best-case property results for different fuel level ranges in figure \ref{fig:permissive_out_of_fuel}.



\begin{figure}
    \begin{center}
        \scalebox{0.6}{\input{fuel_precision}}
    \end{center}
    \caption{This diagram plots the probabilities of running out of fuel, finishing one job, and two jobs with different maximal sensed fuel levels. For example, maximal fuel level = $2$ means that all fuel levels from 2 to 10 will be sensed as fuel level 2.}
    \label{fig:out_of_fuel}
\end{figure}
\begin{figure}
    \begin{center}
        \scalebox{0.6}{\input{permissive_fuel_precision}}
    \end{center}
    \caption{This diagram plots the worst-/best-case probabilities of running out of fuel and finishing two jobs with different ranges for permissive model checking. For example, permissive policy starting range = $2$ means that COOL-MC creates a permissive policy for fuel levels $2-10$.}
    \label{fig:permissive_out_of_fuel}
\end{figure}

==> preliminaries_old.tex <==
A transition system is used to describe the behaviour of an environment. A Discrete-Time Markov Chain (MC) is a transition system with a probability distribution for the successor of each state \cite{baier2008principles}.
\begin{definition}[Discrete-Time Markov Chain (MC)]
    A Discrete-Time Markov chain (MC) is a tuple $\dtmc = (S,P,\iota_{init}, AP, L)$ where
    \begin{itemize}
        \item $S$ is a finite, nonempty set of states,
        \item $P : S \times S \rightarrow [0,1]$ is the transition probability function such that for all states s: $\sum_{s' \in S} P(s,s') = 1$,
        \item $\iota_{init} : S \rightarrow [0,1]$ is the initial distribution such that $\sum_{s \in S} \pi_{init}(s) = 1$,
        \item AP is a set of atomic propositions and $L : S \rightarrow 2^{AP}$ a labeling function.
    \end{itemize}
\end{definition}
A Markov decision process (MDP) is an extension of a Markov chain that introduces nondeterminism, and where the transition Probabilities between the states are determined by the action taken from a given finite set $Act$.
\begin{definition}[Markov Decision Process (MDP]
    A Markov decision process (MDP) is a tuple $\dtmc = (S,P,\iota_{init}, AP, L)$ where $S$ is a finite, nonempty, set of states, Act is a set of actions, $P : S \times A \times S \rightarrow [0,1]$ is the transition probability function such that for all states s: $\sum_{s' \in S} P(s,s') = 1$, $\iota_{init} : S \rightarrow [0,1]$ is the initial distribution such that $\sum_{s \in S} \pi_{init}(s) = 1$, and AP is a set of atomic propositions and $L : S \rightarrow 2^{AP}$ a labeling function.
\end{definition}
A infinite path $\Path = s_0, s_1,... \in S$ such that $P(s_i,s_{i+1}) > 0$ is a state sequence. A finite $\Path = s_0, s_1, ..., s_n$ starts in a state $s_0$ and ends in a state $s_n$. A memoryless deterministic policy $\Policy : S \rightarrow Act$ maps a state $s \in S$ to an action $a \in Act$. Given a policy $\Policy$ and an initial state $s \in S$, $M_P$ becomes purely probabilistic, denoted by $M_{P\Policy}$ \cite{baier2008principles}. A Markov Reward Model (MRM) is a tuple $M_R = (M_C, rew)$ with a Markov chain $M_C$ and $rew : S \times S \rightarrow \Rationals$. For a infinite path $\Path$, we define the long-run average reward in Equation \ref{eq:long_run}.
\begin{equation} \label{eq:long_run}
    \lim_{t \rightarrow \infty} \frac{1}{T} \sum^{T-1}_{t=0} rew(s_t, s_{t+1})
\end{equation}

